Zero-Shot Classification by Logical Reasoning on Natural Language Explanations

Humans can classify data of an unseen category by reasoning on its language explanations. This ability is owing to the compositional nature of language: we can combine previously seen attributes to describe the new category. For example, we might describe a sage thrasher as "it has a slim straight relatively short bill, yellow eyes and a long tail", so that others can use their knowledge of attributes "slim straight relatively short bill", "yellow eyes" and "long tail" to recognize a sage thrasher. Inspired by this observation, in this work we tackle zero-shot classification task by logically parsing and reasoning on natural language expla-nations. To this end, we propose the framework CLORE (Classification by LOgical Reasoning on Explanations). While previous methods usually regard textual information as implicit features, CLORE parses explanations into logical structures and then explicitly reasons along thess structures on the input to produce a classification score. Experimental results on explanation-based zero-shot classification benchmarks demonstrate that CLORE is superior to baselines, which we further show mainly comes from higher scores on tasks requiring more logical reasoning. We also demonstrate that our framework can be extended to zero-shot classification on visual modality. Alongside classification decisions, CLORE can provide the logical parsing and reasoning process as a clear form of rationale. Through empirical analysis we demonstrate that CLORE is also less affected by linguistic biases than baselines.

==> tables/data_variation.tex <==
\begin{table}[t!]
\centering
\small
\linespread{1}

\setlength{\tabcolsep}{1mm}{
\begin{tabular}{l|p{50mm}}

\toprule
Linguistic Bias Type & Description \\
\midrule

Punctuated & Appending punctuation such as ``?'', ``...'' or ``!'' to the input. \\
Hinted & Adding doubting hints in the text, e.g., changing from ``\texttt{odor | pendant}'' to ``\texttt{odor is claimed to be pendant}''. \\
Verbosity & Appending a long meaningless sentence ($\approx$ 30 words) at the end of the input. \\

\bottomrule

\end{tabular}
}

\caption{Types of linguistic biases we adopt. For each linguistic bias type, we program 3 strategies for automatically modifying the inputs.}
% \vspace{-4mm}
\label{tab:data_variation}
\end{table}

==> tables/ecthr_main_results.tex <==
\begin{table*}[t!]
\centering
\small
\linespread{1}

% \setlength{\tabcolsep}{1mm}{
% \resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc}

\toprule

\multirow{2}{*}{\textbf{ECtHR-Explanations}}
& \multicolumn{3}{c}{\textbf{micro-F1}} & \multicolumn{3}{c}{\textbf{macro-F1}} \\
& A-Mean & H-Mean & G-Mean & A-Mean & H-Mean & G-Mean \\
\midrule

T0 (w/o fine-tuning) \\

\midrule

BART-large-MNLI & 0.809 & 0.787 & 0.798 & \textbf{0.477} & \textbf{0.472} & \textbf{0.475} \\
% RoBERTa-base-MNLI \\

Legal-BERT & 0.577 & 0.464 & 0.520 & 0.416 & 0.375 & 0.396 \\
Hierarchical Legal-BERT & 0.779 & 0.756 & 0.768 & 0.449 & 0.447 & 0.448 \\
\model{}$_{Legal-BERT}$ & \textbf{0.823} & \textbf{0.800} & \textbf{0.812} & 0.460 & 0.457 & 0.458 \\
% Hierarchical Legal-BERT & 0.474 & 0.470 & 0.472 \\
% \model{} & \textbf{0.490} & \textbf{0.489} & \textbf{0.490} \\

\bottomrule

\end{tabular}
% }

\caption{Zero-shot classification results on ECtHR-Explanations dataset~\citep{chalkidis2021paragraph}. The A-Mean, H-Mean and G-Mean are the arithmetic, harmonic and geometric averages of ROC-AUC scores across all ECHR articles.
}
\vspace{-4mm}
\label{tab:ecthr_main_results}
\end{table*}

==> tables/execution_evidence.tex <==
\begin{table*}[t!]
\centering
\small
\linespread{1}

\setlength{\tabcolsep}{1mm}{

\NewDocumentCommand{\bluecolor}{ mO{} }{\textbf{\textcolor{blue!60}{#1}}}

\begin{tabular}{m{70mm}|p{30mm}|p{60mm}}

\toprule
\textbf{Input} & \textbf{Logical Structure} & \textbf{Execution Evidence}\\
\midrule


\setlength{\tabcolsep}{0.5mm}{
\ \quad \begin{tabular}[t]{ccccc}
\toprule
\bluecolor{safety} & \bluecolor{person capacity} & \bluecolor{buying cost} & maintenance cost & $\cdots$\\
\midrule
\bluecolor{high} & \bluecolor{4} & \bluecolor{med} & low & $\cdots$
\\
\bottomrule
\\
\end{tabular}
}
&
&
Concept ``with higher safety'' matches 
\textit{\bluecolor{safety|high ... buying cost|med}} with score 0.58 ;
Concept ``and capacity'' matches 
\textit{\bluecolor{safety|high ... buying cost|med}} with score 0.65 ;
\texttt{AND} operator score 0.58; return 0.58
\\

\hline



\begin{tabular}[t]{ccccc}
\toprule
SGPT & SGOT & total bilirubin & \bluecolor{age} & \bluecolor{direct bilirubin} \\
\midrule
33 & 71 & 4\bluecolor{.9} & \bluecolor{65} & \bluecolor{2}.7 \\
\bottomrule
\end{tabular}
&
Label$(X)$ = $\texttt{group above 40}(X)\land \texttt{ensures liver}(X)$
&
\texttt{group above 40} matches \texttt{.9 [SEP] age | 65 [SEP] direct bilirubin | 2} with score 0.56;
\texttt{ensures liver} matches \texttt{.9 [SEP] age | 65 [SEP] direct bilirubin | 2} with score 0.57;
\texttt{AND} operator score 0.56
\\

\hline


\begin{tabular}[t]{ccccc}
\toprule
Club & League & \bluecolor{Venue} & City & ... \\
\midrule
Tulsa Spirit & W\bluecolor{PSL} & \bluecolor{Union} 8th & Broken Arrow & ... \\
\bottomrule
\\
\end{tabular}
& 
Label$(X)$ = $\texttt{league is W}(X)$
&
\texttt{league is W} matches: \texttt{PSL [SEP] Venue | Union} with score 0.72
\\

\hline


\begin{tabular}[t]{m{25mm}m{25mm}c}
\toprule
Association & \bluecolor{Category} & Nominee \\
\midrule
American \bluecolor{Comedy award} & \bluecolor{Funniest Actor in a} Motion Picture & Meg Ryan \\
\bottomrule
\\
\end{tabular}
&
Label$(X)$ = \texttt{association has 'American'}$(X)$
&
\texttt{association has 'American'} matches: \texttt{Comedy award [SEP] Category | Funniest Actor in a} with score 0.69
\\


\bottomrule

\end{tabular}
}

\caption{Examples of logical reasoning evidence. The evidence words are colored in the left column for better visualization.}
\label{tab:execution_evidence}
\end{table*}

==> tables/interpretability.tex <==
\begin{table*}[t!]
\centering
\small
\linespread{1}

\NewDocumentCommand{\blueback}{ mO{} }{\colorbox{blue!15}{#1}}
\NewDocumentCommand{\greenback}{ mO{} }{\colorbox{green!30}{#1}}
\NewDocumentCommand{\bluecolor}{ mO{} }{\textbf{\textcolor{blue!60}{#1}}}

% (a)

\setlength{\tabcolsep}{1mm}{
\begin{tabular}{p{20mm}|p{53mm}|p{80mm}}

% \setlength{\arrayrulewidth}{.3em}

\toprule
\textbf{Class} & \textbf{Natural Language Explanation} & \textbf{Parsed Logical Structure} \\
\midrule

(car-evaluation) vgood
&
\textit{Cars \bluecolor{with higher safety} \greenback{and capacity} are highly acceptable for resale.}
&
($c_{certainty}$=0.74) $~\text{vgood}(X)=\text{\bluecolor{with higher safety}}(X)\land \text{\greenback{and capacity}}(X)$
% $ ~\text{function}_1$ = \textit{Exist}(\texttt{\bluecolor{with higher safety}}; X);
% $\text{function}_2$ = \textit{Exist}(\texttt{\greenback{with higher safety and capacity}}; X);
% $\text{function}_3$ = And($\text{function}_1$, $\text{function}_2$; X);
% return $\text{function}_3$(X)
\\

\bottomrule

\end{tabular}
}

\vspace{0.3cm}

% (b)
\begin{tabular}{p{85mm}|p{70mm}}
\toprule
\textbf{Input} & \textbf{Execution Evidence}\\
\midrule
% \texttt{SGPT | 33 [SEP] SGOT | 71 [SEP] total bilirubin | 4\bluecolor{.9 [SEP] age | 65 [SEP] direct bilirubin | 2}.7 [SEP]}
\setlength{\tabcolsep}{0.5mm}{
\ \quad \begin{tabular}[t]{ccccc}
\toprule
% \greenback{\bluecolor{safety}} & \greenback{\bluecolor{person capacity}} & \greenback{\bluecolor{buying cost}} & maintenance cost & luggage boot size \\
% \midrule
% \greenback{\bluecolor{high}} & \greenback{\bluecolor{4}} & \greenback{\bluecolor{med}} & low & med
\greenback{\bluecolor{safety}} & \greenback{\bluecolor{person capacity}} & \greenback{\bluecolor{buying cost}} & maintenance cost & $\cdots$\\
\midrule
\greenback{\bluecolor{high}} & \greenback{\bluecolor{4}} & \greenback{\bluecolor{med}} & low & $\cdots$
\\
\bottomrule
\\
\end{tabular}
}
&
% function$_1$(X) = \textit{Exist}(\texttt{group above 40}; X);
% function$_2$(X) = \textit{Exist}(\texttt{ensures liver}; X);
% function$_3$(X) = And(function$_1$, function$_2$; X);
% return function$_3$(X)
% &
% function$_1$(X)=0.58 attends to: \texttt{\bluecolor{safety|high ... buying cost|med}};
% function$_2$(X)=0.65 attends to: \texttt{\greenback{safety|high ... buying cost|med}};
% function$_3$(X)=0.58; return 0.58 (\textbf{positive}) \\
Concept ``with higher safety'' matches 
\textit{\bluecolor{safety|high ... buying cost|med}} with score 0.58 ;
Concept ``and capacity'' matches 
\textit{\greenback{safety|high ... buying cost|med}} with score 0.65 ;
\texttt{AND} operator score 0.58; return 0.58\\
\bottomrule
\end{tabular}

\vspace{3mm}

\begin{tabular}[t]{c|c|c}
\toprule
Ground-truth label: \textbf{positive} & \model{} prediction: \textbf{positive} & ExEnt prediction: \textbf{negative} \\
\bottomrule
\end{tabular}

\caption{A visualization example of parsed logical structure on an explanation and \model{}'s reasoning evidence on an input from CLUES dataset.
The blue font and green background indicate two attributes (``higher safety'' and ``capacity'') involved in this example.
% \zhenhailong{\sout{add a brief description of the task/dataset this example comes from?}}
% \zhenhailong{\sout{add description of the meaning of the text color and the background color?}} \yi{where is this table referenced in this page?}
% \chihan{oh it is in page 6-7 actually. I agree the figure is better repositioned.}
}
\vspace{-4mm}
\label{tab:interpretability}
\end{table*}

==> tables/program_semantics.tex <==
\begin{table}[t!]
\centering
\small
\linespread{1}

\setlength{\tabcolsep}{1mm}{
\begin{tabular}{c|ccp{40mm}}
\toprule

Type & \#Arg. & w/ Content & Meaning \\

\midrule

Select & 0 & True & selecting input words related to \textit{content} \\

% Relate & 1 & True & selecting input words related to \textit{content} about the argument \\

And & 2 & False & get intersection of two arg. \\
Or & 2 & False & get union of two arg. \\
Not & 1 & False & get complementary of arg. \\
End & 0 & False & terminate the program \\

\bottomrule
\end{tabular}}

\caption{Semantics of the module types. The second column displays the number of arguments accepted by this type of module. The third column indicates whether the module has a content or not.}
% \vspace{-6mm}
\label{tab:program_semantics}
\end{table}

==> tables/quantifier_extraction.tex <==
\begin{table}[t!]
\centering
\small
\linespread{1}

% \setlength{\tabcolsep}{1mm}{
\begin{tabular}{c|c}
\toprule
Quantifier & Rule for detecting the quantifier \\
\midrule
usually & definition contains \textit{usually} or \textit{Usually} \\
% always & definition contains \textit{always} \\
generally & definition contains \textit{generally} or \textit{Generally} \\
often & definition contains \textit{often} or \textit{Often} \\
likely & definition contains \textit{more likely} or \textit{most likely} \\
most & definition contains \textit{most} or \textit{Most} \\
majority & definition contains \textit{majority} \\
frequently & definition contains \textit{frequently} or \textit{Frequently} \\
\bottomrule
\end{tabular}
% }

\caption{Rules for detecting quantifiers in definitions.\xd{i think this table is spurious, if the draft is over 7 pages, rm it and only mention we sue "usually, generally, ..." in main text.}}
% \vspace{-4mm}
\label{tab:quantifier_extraction}
\end{table}
